A Process Algebra for Wireless Mesh Networks

We propose a process algebra for wireless mesh networks that combines novel treatments of local broadcast, conditional unicast and data structures. In this framework, we model the Ad-hoc On-Demand Distance Vector (AODV) routing protocol and (dis)prove crucial properties such as loop freedom and packet delivery.

==> fig/ex_aodv_1.tex <==
\pspicture(-10,-10)(10,10)

%%  NODES  %%
   \cnode(1.0,0.0){0.2}{d}
   \rput(1.0,0.0){$d$}

   \cnode(0.0,-1.0){0.2}{b}
   \rput(0.0,-1.0){$b$}

   \cnode(-1.0,0.0){0.2}{s}
   \rput(-1.0,0.0){$s$}

   \cnode(0.0,1.0){0.2}{a}
   \rput(0.0,1.0){$a$}


%%  EDGES  %%
   \ncline{s}{a}
   \ncline{a}{b}
   \ncline{b}{d}
   \ncline{s}{b}
   \ncline{a}{d}

%%  MSGS  %%

\endpspicture


==> fig/ex_aodv_2.tex <==
\pspicture(-10,-10)(10,10)

%%  NODES  %%
   \cnode(1.0,0.0){0.2}{d}
   \rput(1.0,0.0){$d$}

   \cnode(0.0,-1.0){0.2}{b}
   \rput(0.0,-1.0){$b$}

   \cnode(-1.0,0.0){0.2}{s}
   \rput(-1.0,0.0){$s$}

  \cnode(0.0,1.0){0.2}{a}
   \rput(0.0,1.0){$a$}

%%  EDGES  %%
%   \ncline{s}{a}
%   \ncline{a}{b}
%   \ncline{b}{d}
%   \ncline{s}{b}
%   \ncline{a}{d}

%%  MSGS  %%
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt]{->}{s}{a}
   \aput[1pt]{:U}{\tiny RREQ\ }
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt]{<-}{b}{s}
   \aput[1pt]{:D}{\tiny RREQ\ }
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt]{->}{a}{d}
   \aput[1pt]{:U}{\tiny RREQ\ }
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt]{<-}{d}{b}
   \aput[1pt]{:D}{\tiny RREQ\ }
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=1.25pt]{->}{a}{b}
   \aput[1pt]{:U}{\tiny RREQ\ }
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=1.25pt]{->}{b}{a}
   \aput[1pt]{:D}{\tiny RREQ\ }

\endpspicture


==> fig/ex_aodv_3.tex <==
\pspicture(-10,-10)(10,10)

%%  NODES  %%
   \cnode(1.0,0.0){0.2}{d}
   \rput(1.0,0.0){$d$}

   \cnode(0.0,-1.0){0.2}{b}
   \rput(0.0,-1.0){$b$}

   \cnode(-1.0,0.0){0.2}{s}
   \rput(-1.0,0.0){$s$}

   \cnode(0.0,1.0){0.2}{a}
   \rput(0.0,1.0){$a$}

%%  EDGES  %%
   %\ncline{s}{a}
   \ncline{a}{b}
   \ncline{b}{d}
   \ncline{s}{b}
   %\ncline{a}{d}

%%  MSGS  %%
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt]{<-}{a}{d}
   \aput[1pt]{:U}{\tiny \ RREP}
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt]{<-}{s}{a}
   \aput[1pt]{:U}{\tiny \ RREP}

\endpspicture

